Robust Training of Federated Models with Extremely Label Deficiency

Federated semi-supervised learning (FSSL) has emerged as a powerful paradigm for collaboratively training machine learning models using distributed data with label deficiency. Advanced FSSL methods predominantly focus on training a single model on each client. However, this approach could lead to a discrepancy between the objective functions of labeled and unlabeled data, resulting in gradient conflicts. To alleviate gradient conflict, we propose a novel twin-model paradigm, called Twin-sight, designed to enhance mutual guidance by providing insights from different perspectives of labeled and unlabeled data. In particular, Twin-sight concurrently trains a supervised model with a supervised objective function while training an unsupervised model using an unsupervised objective function. To enhance the synergy between these two models, Twin-sight introduces a neighbourhood-preserving constraint, which encourages the preservation of the neighbourhood relationship among data features extracted by both models. Our comprehensive experiments on four benchmark datasets provide substantial evidence that Twin-sight can significantly outperform state-of-the-art methods across various experimental settings, demonstrating the efficacy of the proposed Twin-sight.

==> main_paper/Pre.tex <==
\section{Preliminary}
In general, FL tends to train a global model parameterized by $w$ with $K$ participants collaboratively. In other words, the objective function of the global model $\mathcal{J}(w)$ is composed of the local function over all participants' data distribution:
\begin{equation}
\label{eq:normal_obj}
        \min_{w} \mathcal{J}(w) = \sum_{k=1}^{K} \beta_k \mathcal{J}_{k}(w_k).
\end{equation}
where $\beta_k$ determine the weight of $k$-th client's contribution. Considering the $k$-th client possesses a local private dataset denoted by $\mathcal{D}_k$, drawn from the distribution $P_k$. 

In FSSL, a typical scenario involves $M$ clients with fully-labeled data, while the remaining $T$ clients have unlabeled data. The set of all clients $C = \{c_k\}^{K}_{k=1}$ can be divided into two subsets, $C^{L}=\{c_m\}^{M}_{m=1}$ and $C^{U}=\{c_t\}^{T}_{t=1}$, corresponding to the clients with labeled and unlabeled data, respectively. The dataset of $m$-th client in $C^{L}$ is $\mathcal{D}_{m}^{l} = \{ (\textbf{x}_{m}^{i}, y_{m}^{i} )\}^{N_m}_{i=1}\sim P_m$ and $\mathcal{D}_t^{U} = \{ (\textbf{u}_{t}^{i} )\}^{N_t}_{i=1}\sim P_{t}$ denotes the unlabeled data $i$-th sample witout annotation in client $c_t$'s private dataset.

\subsection{Dual-model Paradigm}
Revisit the conventional FSSL framework, the local objective function on labeled data can be formulated as:
\begin{equation}
    \mathcal{J}_{m}(w_{m}) \triangleq \mathbb{E}_{(x,y) \sim P_m} \ell(w_m;x, y),
\end{equation}
where $\mathbb{E}$ is the expectation of loss function on data distribution $P_m$ and $\ell$ is the cross-entropy loss. To facilitate the unlabeled data, some semi-supervised 

==> main_paper/ProDef.tex <==
\section{\method Problem Definition}

